Binary Classification with Karmic, Threshold-Quasi-Concave Metrics

Complex performance measures, beyond the popular measure of accuracy, are increasingly being used in the context of binary classification. These complex performance measures are typically not even decomposable, that is, the loss evaluated on a batch of samples cannot typically be expressed as a sum or average of losses evaluated at individual samples, which in turn requires new theoretical and methodological developments beyond standard treatments of supervised learning. In this paper, we advance this understanding of binary classification for complex performance measures by identifying two key properties: a so-called Karmic property, and a more technical threshold-quasi-concavity property, which we show is milder than existing structural assumptions imposed on performance measures. Under these properties, we show that the Bayes optimal classifier is a threshold function of the conditional probability of positive class. We then leverage this result to come up with a computationally practical plug-in classifier, via a novel threshold estimator, and further, provide a novel statistical analysis of classification error with respect to complex performance measures.

==> binary_search.tex <==
% analysis of binary search
\subsection{Convergence rate of binary search}
\label{app:proof_binary_search}

 The proof of Lemma~\ref{th:binary_guarantee} relies on the following general lemma.
 \begin{lemma}
 If $\cV_\eta(\delta, \bP)$ has a unique maximizer $\delta^*$. Let $\hat{\delta}$ be the output of Algorithm~\ref{alg:binary_search} with input conditional probability function $\heta$. If there exists constants $L_v,c_1,\gamma$ such that
 \begin{enumerate}
 \item $\cV_{\heta}(\delta,\bP)$ is $L_v$-Lipschitz continuous for any $\heta$ satisfying Assumption~\ref{ass:eta_injective};
 \item If $|\delta-\delta^*|\ge \gamma$, then $\sign{\cV'_\eta(\delta,\bP)} = \sign{\cV'_{\heta}(\delta,\bP_n)}$.
 \item If $|\delta-\delta^*| < \gamma$, then $|\cV'_\eta(\delta,\bP_n)|\le c_1\gamma$.
 \end{enumerate}
 Then with the tuning parameter $\epsilon_0$ in Algorithm~\ref{alg:binary_search} set as $\epsilon_0 = c_1\gamma^2/L_v$, we have
 \bas{
 \cU(\sign{\heta(x) - \delta^*},\bP)  - \cU(\sign{\heta(x) - \hat{\delta}},\bP)  \le 3c_1\gamma^2
 }
 \label{lem:binary_convergence_general}
 \end{lemma}
 The intuition for the conditions is straightforward. We hope the empirical evaluated sign to be equal to the population value of the sign when the threshold is far from the optimum, hence the update has the correct direction. And the objective function is also smooth enough around the optimum, so that the cumulative difference can be bounded.

\begin{proof}[Proof of Lemma~\ref{th:binary_guarantee}]
It suffices to check the three conditions in Lemma~\ref{lem:binary_convergence_general}. Recall $v(\delta) = (-\delta,-(1-\delta),\delta,1-\delta)$.
%Take $\gamma = \max\{\frac{\log a_n}{a_n},\frac{\log n}{n}\}$.
\paragraph{1. $\cV_\eta(\delta,\bP)$ is Lipschitz continuous}
First by Assumption~\ref{ass:eta_injective}, $p_\eta(\cdot)$ is bounded everywhere.
If $\cG(\bC) = \frac{\baa^T\bC}{\bb^T\bC}$, then $\cV'_{\heta}(\delta,\bP)=\frac{(\bb^T\bC)(\baa^Tv(\delta))-(\baa^T\bC)(\bb^Tv(\delta))}{(\bb^T\bC)^2}\cdot p_\eta(\delta)$. Note $|\bb^T\bC|>0$, and $\bC$ is on a compact set, hence there exists constant $c$ such that $|\bb^T\bC|\ge c$. Therefore, $|\cV'_{\heta}(\delta,\bP)|$ is bounded by some constant $L_v$.

If $\cG$ is concave and twice continuously differentiable, $\cV'_{\heta}(\delta,\bP)=\nabla \cG(\bC)^Tv(\delta)p_\eta(\delta)$. Due to the fact that $\nabla \cG(\bC)$ is continuous, we know it has an upper bound on confusion matrix domain $[0,1]^4$. Hence there exists constant $L_v$ such that $\cV_{\heta}(\delta,\bP)$ is $L_v$-Lipschitz continuous.

\paragraph{2. $\Phi_\eta(\delta,\bP)=\Phi_{\heta}(\delta,\bP_n)$ when $|\delta-\delta^*|\ge \gamma$}
Recall the function $H$ defined in the proof of Corollary~\ref{prop:quasi-concave}.
$\Phi_\eta(\delta,\bP) = \sign{\cV'_\eta(\delta,\bP)} = \sign{H_\eta(\delta,\bP)}$. Hence it suffices to show that $|H_\eta(\delta,\bP)| \ge |H_\eta(\delta,\bP)-H_{\heta}(\delta,\bP_n)|$.

Given $\hat{\eta}$ and $\delta$ fixed, we have $\bE_X 1(\hat{\eta}(X)>\delta)\eta(X) = \tp(\sign{\hat{\eta}(X)-\delta},\bP)$. Note that $1(\hat{\eta}(X)>\delta)\eta(X) - \bE 1(\hat{\eta}(X)>\delta)\eta(X)$ is mean zero and absolutely bounded by 2. Hence by Bernstein's inequality, for $\epsilon>0$, 
\ba{
P(|\tp(\sign{\hat{\eta}(x) - \delta^*},\bP_n)-\tp(\sign{\hat{\eta}(x) - \delta^*},\bP)|>\epsilon)\le C_1\exp(-C_2n\epsilon^2)
\label{eq:tp_concentration}
}
Similarly we get that for the entire confusion matrix, with probability greater than $1-n^{-c_1}$,
\bas{
\| \bC(\sign{\heta(X) - \delta},\bP)  - \bC(\sign{\heta(X) - \delta},\bP_n)\| \le c_2\sqrt{\frac{\log n}{n}}
}
By similar reasoning as the above paragraph, there exists a constant $c_3$ such that 
\ba{
|H_{\heta}(\delta,\bP) - H_{\heta}(\delta,\bP_n)| \le c_3\|\bC(\sign{\heta-\delta},\bP) - \bC(\sign{\heta-\delta},\bP_n)\|
\label{eq:phi_lipschitz}
}
for both linear fractional functions and concave functions.
Hence, there exists $c_4 \in \bR$ such that 
\ba{
P \left( |H_{\heta}(\delta,\bP) - H_{\heta}(\delta,\bP_n) |\ge c_4\sqrt{\frac{\log n}{n}} \right) \le n^{-1}
\label{eq:H_heta_p_pn}
}

On the other hand, by Lemma~\ref{thm:confusion_with_same_threshold}, we have
\bas{
\| \bC(\sign{\heta(X) - \delta},\bP)  - \bC(\sign{\eta(X) - \delta},\bP)\| \le c_5\bE_X|\heta-\eta| 
}
Hence by Lipschitzness of $H$ and Assumption~\ref{ass:eta_concentration}, we have with probability greater than $1-a_n^{-1}$,
\ba{
|H_{\heta}(\delta) - H_{\eta}(\delta)| \le c_5\sqrt{\frac{\log a_n}{a_n}}
\label{eq:H_heta_eta}
}
For concave functions, by Eq.~\eqref{eq:H_prime_bounded_from_below}, $|H'_\eta(\delta,\bP)|\ge C_B$. For linear fractional functions, by working out the derivative of $H$, we know it is bounded from below. There exists $c_6>0$, such that $\forall |\delta-\delta^*|\ge \gamma$, $|H_\eta(\delta)|\ge c_6 \gamma$. For $\gamma\ge \frac{c_4}{c_6}\sqrt{\frac{\log n}{n}}+\frac{c_5}{c_6}\sqrt{\frac{\log a_n}{a_n}})$, by Eqs.~\eqref{eq:H_heta_p_pn} and \eqref{eq:H_heta_eta}, 
\bas{
|H_\eta(\delta,\bP)| \ge |H_\eta(\delta,\bP)-H_{\heta}(\delta,\bP_n)|
}
This implies all the empirically evaluated signs for $|\delta-\delta^*|\ge \gamma$ are correct, i.e., $\Phi_\eta(\delta,\bP) = \Phi_{\heta}(\delta,\bP_n)$.

\paragraph{3. Smoothness around the optimum}
\bas{
|\cV'_{\heta}(\delta,\bP)|\le |H_{\heta}(\delta,\bP)|\cdot \max_{\delta}p_{\heta}(\delta)
}
The gradient of $H$ is a continuous function defined on a compact domain, and is bounded. Hence $H_{\eta}(\delta,\bP)$ is $\ell_0$-Lipschitz continuous. We know that $H_{\eta}(\delta^*,\bP)=0$. So by Eq.~\eqref{eq:H_heta_eta},
\bas{
H_{\heta}(\delta,\bP)\le& |H_{\heta}(\delta,\bP)-H_{\eta}(\delta,\bP)|+|H_{\eta}(\delta,\bP)|\\
\le & c_5\sqrt{\frac{\log a_n}{a_n}}+\ell_0\gamma
}
Meanwhile, $\max_{\delta}p_{\heta}(\delta)$ is bounded by Assumption~\ref{ass:eta_injective}. Take $\gamma=c_7\frac{\log \tilde{n}}{\tilde{n}}$ with large enough constant $c_7$, all three conditions in Lemma~\ref{lem:binary_convergence_general} are satisfied.

\end{proof}

\subsection{Rate of convergence for the two-step plug-in classifier with binary search}
\begin{proof}[Proof of Theorem~\ref{thm:final_gen_bound}]
Assume the classifier returned is $\hat{f}(x)=\sign{\hat{\eta}(x)-\delta}$, where $\hat{\eta}$ is learned with the first $n_1$ samples $\{X_i^{(1)},Y_i^{(1)}\}$, and $\delta$ is returned by Algorithm~\ref{alg:binary_search} with $n_2$ samples. 
By Lemma~\ref{th:conv_rate_deltastar},
\bas{
| \cU(f^*,\bP)-\cU(\heta-\delta^*,\bP)| \le C_1a_{n_1}^{-\frac{1+\alpha}{2}}
}
By Assumption~\ref{ass:conv_of_thres_finding} and Lemma~\ref{th:binary_guarantee}, with probability at least $1-\min\{a_{n_2},n_2\}^{-c}$, 
\bas{
|\cU(\heta-\delta^*,\bP)-\cU(\heta-\hat{\delta},\bP)| \le C_2\frac{\log (\min\{a_{n_2},n_2\})}{\min\{a_{n_2},n_2\}}
}
Taking $n_1=n_2=\frac{n}{2}$, we have with probability at least $1-\min\{a_{n},n\}^{-c}$,
\bas{
\cU(f^*,\bP) - \cU(\hat{f},\bP) \le& | \cU(\sign{\eta-\delta^*},\bP)-\cU(\heta-\delta^*,\bP)|+|\cU(\heta-\delta^*,\bP)-\cU(\heta-\hat{\delta},\bP)|\\
\le& C_1 a_{n_1}^{-\frac{1+\alpha}{2}} + C_2 \max \left\{ \frac{\log a_{n_2}}{a_{n_2}},\frac{\log n_2}{n_2}  \right\}\\
\le & C_3 \max\left\{ \frac{\log n}{n},\frac{\log a_n}{a_n},a_{n}^{-\frac{1+\alpha}{2}}  \right\}
}

\end{proof}

==> quasi_concavity.tex <==
\section{Proofs in Section~\ref{sec:estimation}}
\label{sec:proof_quasi_concave}



\begin{proof}[Proof of Lemma~\ref{lem:binary_convergence_general}]

%Denote $\Delta = c_1 \gamma$, $\delta_1 = \sup\{\delta: H_\eta(\delta)\ge \Delta\}$ and $\delta_2 = \inf \{\delta: H_\eta(\delta)\le -\Delta\}$. It is easy to see that $\delta_1<\delta_2$ and $|\delta_1-\delta_2|\le 2\gamma$. 
By the update rule of Algorithm~\ref{alg:binary_search} and condition 2, we have $\hat{\delta}\in (\delta^*-\gamma-\frac{\epsilon_0}{2},\delta^*+\gamma+\frac{\epsilon_0}{2})$. 

Now the difference in utility can be bounded as follows.
\ba{
&|\cU(\sign{\heta(X) - \delta^*},\bP)   - \cU(\sign{\heta(X) - \hat{\delta}},\bP)| \nonumber\\
\le & \underbrace{\left| \int_{\delta^*-\gamma-\frac{\epsilon_0}{2}}^{\delta^*-\gamma} \cV'_{\heta}(\delta,\bP) d\delta\right|+ \left|\int_{\delta^*+\gamma}^{\delta^*+\gamma+\frac{\epsilon_0}{2}} \cV'_{\heta}(\delta,\bP) d\delta \right|}_{\rom{1}}+ \underbrace{\left|\int_{\delta^*-\gamma}^{\delta^*+\gamma} \cV'_{\heta}(\delta,\bP) d\delta \right|}_{\rom{2}}. \label{eq:u_decomposition}
}
By condition 1, $\rom{1} \le  L_v\epsilon_0$.
Eq.~\eqref{eq:u_decomposition} can be bounded by the flatness of $\cV_{\heta}(\delta)$. By condition 3, we have,
\ba{
& \left| \int_{\delta^*-\gamma}^{\delta^*+\gamma} \cV'_{\heta}(\delta,\bP) d\delta \right| \le  \int_{\delta^*-\gamma}^{\delta^*+\gamma} |\cV'_{\heta}(\delta,\bP)| d\delta \le 2\gamma\cdot c_1\gamma = 2c_1\gamma^2.
\label{eq:u_flat_bound}
}
Taking $\epsilon_0=\frac{c_1}{L_v}\gamma^2$ and combining Eqs.~\eqref{eq:u_decomposition} and \eqref{eq:u_flat_bound}, we have
\bas{
& \cU(\sign{\heta(X) - \delta^*},\bP)  - \cU(\sign{\heta(X) - \hat{\delta}},\bP) \le 3c_1\gamma^2.
}
\end{proof}



==> threshold_search.tex <==
\subsection{Threshold Search}
\label{sec:thres_search}

%Different from the 0-1 loss classification, for optimizing the Bayes classifier, one needs not only to estimate the conditional probability, but also the optimal threshold. 








%The proof is a combination of Proposition~\ref{th:conv_rate_deltastar} and Proposition~\ref{th:binary_guarantee} and is presented in Appendix~\ref{app:proof_binary_search}.



